IMUGPT 2.0: Language-Based Cross Modality Transfer for Sensor-Based Human Activity Recognition

One of the primary challenges in the field of human activity recognition (HAR) is the lack of large labeled datasets. This hinders the development of robust and generalizable models. Recently, cross modality transfer approaches have been explored that can alleviate the problem of data scarcity. These approaches convert existing datasets from a source modality, such as video, to a target modality (IMU). With the emergence of generative AI models such as large language models (LLMs) and text-driven motion synthesis models, language has become a promising source data modality as well as shown in proof of concepts such as IMUGPT. In this work, we conduct a large-scale evaluation of language-based cross modality transfer to determine their effectiveness for HAR. Based on this study, we introduce two new extensions for IMUGPT that enhance its use for practical HAR application scenarios: a motion filter capable of filtering out irrelevant motion sequences to ensure the relevance of the generated virtual IMU data, and a set of metrics that measure the diversity of the generated data facilitating the determination of when to stop generating virtual IMU data for both effective and efficient processing. We demonstrate that our diversity metrics can reduce the effort needed for the generation of virtual IMU data by at least 50%, which open up IMUGPT for practical use cases beyond a mere proof of concept.

==> sections/filter/main.tex <==
\section{Filtering out incorrectly generated motion sequences}
\label{sec: motion_filter}

\input{figure/motion_filter}

In order to address one of the limitations of Leng et al.'s system \cite{leng2023generating} — the motion synthesis model generates motion sequences that do not accurately describe the intended activity — we propose a pipeline called the 'motion filter' that can filter out incorrectly generated motion sequences.

\autoref{fig:motion_filter} illustrates the operation of the motion filter. To determine if a given motion sequence accurately portrays the activity of interest, the sequence generated by the motion synthesis model is first processed by a motion captioning model \cite{jiang2023motiongpt}. This model outputs a textual description of the motion sequence. The resulting motion caption is then evaluated by a LLM, which provides a binary 'yes' or 'no' answer indicating whether the caption accurately describes the specified activity. This output from the LLM enables us to filter out any incorrectly generated motion sequences.

We hypothesize that incorrectly generated motion sequences will detrimentally affect the downstream classifier's performance, as the virtual IMU data extracted from these sequences could be misinterpreted as noise. Therefore, we postulate that removing these sequences should enhance the classifier's effectiveness. The subsequent sections detail the two components of the motion filter.\hyeok{This last paragraph is redundant.}

\subsection{Motion Captioning}
\subsubsection{Model Architecture}
 The motion captioning task, also called the motion-to-text task, refers to generating a text description for a given human motion sequence. TM2T \cite{Guo2022tm2t} and MotionGPT \cite{jiang2023motiongpt} are two recently proposed model for the motion captioning task. In this work, we use MotionGPT as our motion captioning model to caption the generated motion sequences due to its superior performance. MotionGPT is a motion-language model that fuses large amount of language data and motion data to handle numerous motion-relevent tasks such as text-driven motion
synthesis, motion captioning, motion prediction, and motion in-between. 

To caption a given input motion sequence of length $M$ frames $m^{1:M} = \{x_i\}_{i=1}^M$, the motion sequence is first encoded into $L$ discrete motion tokens $z^{1:L} = \bm{\varepsilon}(m^{1:M}) = \{z_i\}_{i=1}^L, L = M/l$, using a motion encoder $\bm{\varepsilon}$, where $l$ is the temporal downsampling rate on motion length. The motion encoder is part of a motion tokenizer that is based on the Vector Quantized Variational Autoencoders (VQ-VAE) architecture \cite{oord2017vq-vae}. This allows the motion sequence to be represented as a language. The motion encoder consists of two parts: 1D convolutions and quantization. In the first part, 1D convolution layers are applied to the motion sequence $m^{1:M}$ along the time dimension to obtain the latent vectors $\hat{z}_{1:L}$. Through discrete quantization, the latent vectors are converted into code indices using a learnable codebook  $Z = \left\{ z_i \right\}_{i=1}^K \subset \mathbb{R}^d$ with $K$ latent embedding vectors of dimension $d$. During quantization, each latent vector is replaced with the nearest vector in $Z$, which minimizes the Euclidean distance:
\begin{equation}
z_i=\arg\min_{z_k\in Z}\left\|\hat{z}_i-z_k\right\|_2
\end{equation}
$z_i$ is the quantized latent vector. The code indices corresponding to the quantized latent vectors in the codebook are called motion tokens, which can be seen as the vocabulary for human motion.

In addition to taking in a motion sequence as input, MotionGPT also takes in a textual prompt describing the specific task to be performed, in this case, motion captioning. Similar to the input motion sequence, the input textual prompt is tokenized using the text encoder of a pretrained text tokenizer, SentencePiece \cite{kudo2018sentencepiece}, with a vocabulary of $K_t$ text tokens. The text vocabulary $V_t = \{v_t^i\}_{i=1}^{K_t}$ is combined with the motion vocabulary $V_m = \{v_{m}^i\}_{i=1}^{K_m}$, which includes motion tokens and additional special tokens like those indicating the start and end of a motion sequence, to form the unified vocabulary $V = \{V_t, V_m\}$ of a language model. The tokens/words within the new vocabulary can represent text, human motion, or a mixture of the two. This flexibility in representation allows MotionGPT to use both text and motion as input and output to accomplish a range of motion-related tasks with a single model.

The sequence of text and motion tokens $X_s = \{x_s^i\}_{i=1}^N
$, $x_s \in V$, are passed to a transformer-based language model as input. The language model generates a sequence of output tokens $X_t = \{x_t^i\}_{i=1}^L
$, in an autoregressive manner, and it is trained using the following loss function

\begin{equation}
\mathcal{L}_{LM} = -\sum_{i=0}^{L_t-1} \log p_\theta (x_t^i | x_t^0, \ldots , x_t^{i-1}, x_s)
\end{equation}
Lastly, the sequence of output tokens are decoded using a text decoder and a motion decoder to recover the output texts, motion caption in this case, and motion (none for the motion caption task). 


\subsubsection{Implementation} The codebook size of the motion encoder is set to $Z \in \mathbb{R} ^{512x512}$. Additionally, the motion encoder uses a temporal downsampling rate of 4. T5 \cite{Colin2020t5} is chosen as the transformer-based language model with 12 layers in both the encoder and decoder. The model is trained on the HumanML3D dataset \cite{Guo_2022_CVPR}, a dataset containing large amounts of human motion capture data along with the corresponding textual descriptions, using the AdamW optimizer. 


\input{figure/motion_filter_LLM}

\subsection{Activity Classification Using Large Language Models}
\hyeok{activity classification sounds misleading. Isn't this just a filtering?}

The emergence of Large Language Models (LLMs) such as GPT-3 \cite{brown2020gpt3}, GPT-4 \cite{openai2023gpt4}, PaLM 2 \cite{anil2023palm}, and LLama 2 \cite{touvron2023llama} has revolutionized the field of natural language processing (NLP) due to their impressive capabilities in various NLP tasks, made possible by their massive training corpora. The success of LLMs has also attracted attention in other fields, where they are integrated with an array of AI models, with the LLMs facilitaing the interaction between the AI models and the end-user \cite{shen2023hugginggpt, wu2023visual}. Additionally, in a recent study, Athanasiou et al. \cite{SINC:ICCV:2022} discovered that motion and activity information is encoded within LLMs, demonstrating that they could use GPT-3 to identify the body parts involved in different activities. Inspired by this result, we apply LLMs to the problem of activity classification in this work, utilizing the motion caption by the motion caption model \cite{jiang2023motiongpt}.
\hyeok{This sounds more like background. move to related work.}

\subsubsection{Problem Definition} The problem is framed as a binary classification task where the input is a textual description $m$, the motion caption, of a human motion sequence, along with a specific activity of interest $a$. The output is a binary label $y \in \{ 0,1\}$ that indicates whether the input textual description accurately depicts a person performing the activity in question. Let $\mathcal{M}$ represent the space of all possible textual motion captions, and let $\mathcal{A}$ represent the set of all predefined activities of interest. We seek to learn a function $f$ that maps a pair consisting of a motion caption and an activity to a binary label:  $ f: \mathcal{M} \times \mathcal{A} \rightarrow \{0, 1\}$. The goal of $f$ is to determine whether a given motion caption $m \in \mathcal{M}$ correctly describes a person performing a given activity $a \in \mathcal{A}$. With conventional supervised methods in NLP, learning such a function would require large amounts of training data containing motion captions for specific activities. However, collecting such a dataset would be extremely time consuming and practically infeasible. 

\subsubsection{LLM Prompting} Hence, we decided to turn to LLMs for this problem as they have shown impressive performances on zero-shot NLP tasks. Through our early explorations, we believe the function $f$ has been implicit learned by the LLMs during the training process due to the massive training corpus as we found that the LLMs have a good understanding of the correspondence between the motion descriptions and activities. 

To obtain labels from the LLM, we first assign it a task via a system message. In this message, the LLM is asked to provide 'yes' or 'no' responses, indicating whether the user-provided motion captions describe the specified activity accurately. Using this system message helps the LLM understand its role and significantly reduces post-processing effort. Without this message, we found that the LLM often produces additional, miscellaneous texts unrelated to the task. After setting up the system message, we provide the specified activity name and a list of motion captions, with 10 captions per prompt, to the LLM. The LLM then outputs 'yes' or 'no' for each caption. A 'yes' response indicates that the caption correctly describes someone performing the specified activity, and 'no' indicates otherwise. We use the LLM's responses to filter out incorrectly generated motion sequences. 

This approach is a zero-shot task for the LLM, as we do not provide any example captions and labels for it to learn from. We detail the exact prompts used, along with some example motion captions and the corresponding labels generated by the LLM, in \autoref{fig:motion_filter_llm}. For the labels shown in \autoref{fig:motion_filter_llm}, we used GPT-4 \cite{openai2023gpt4} as our LLM. It's important to note that the LLM is not infallible; for example, it incorrectly labeled the caption 'a person jogs in place then stops' as 'no' for the running activity.  We evaluate how well the proposed motion filter can filter out incorrectly generated motion sequences in section \ref{sec: motion_filter_eval}. 




==> sections/ideas/main.tex <==

% \vspace{-0.1in}
% \section{ideas}

% \begin{itemize}
%     \item How to quantitatively measure the diversity of the text prompts? 
%         \begin{itemize}
%             \item HAID \cite{bai2023executives} used for measuring the semantic difference between texts answers from human and LLMs for earning calls. Could come up with something similar\\
%             (Uses BERT and Word2vec embeddings to compute the cosine similarity between two pieces of text.) 
%             \item Use 2 LLMs, 1 will be used to generate the textual descriptions. Then feed the generated textual descriptions into another LLM and ask that LLM to output a value for how diverse the textual descriptions are. 
%             \item Brute force method, Keep generating textual descriptions until the downstream classifier performance no longer improves. However, this lacks novelty and does not provide much insights.
%             \item Use 2 LLMs, 1 will generate textual descriptions for a specific activity. For each generated textual description, ask another LLM what activity the generated textual descriptions corresponds to. 
%             \item Tokenize the textual descriptions using a tokenizer (eg. OpenAI's tokenizer) and run a cluster algorithm (K-menas) to cluster the text embeddings. 
%             \item Take a deep dive into the NLP fields to see what existing metrics are there. E.g. Bleu \cite{papineni2002bleu}, Cider \cite{vedantam2015cider}, Rouge \cite{lin2004rouge}, Bertscore \cite{zhang2019bertscore}
%         \end{itemize}
%     \item Experiment with different LLMs to see if there is a difference between the diversity of the textual descriptions generated by each LLM 
%         \begin{itemize}
%             \item GPT 3.5 (Used in original paper)
%             \item GPT 4
%             \item Bard
%             \item Llama 2 (Various parameters)
%             \item Open Assistant
%             \item ...
%         \end{itemize}

%     \item Experiment with adding additional parameters to the generated text and see if it makes a difference in the generated motion
%         \begin{itemize}
%             \item Age (e.g. children, young adults, middle age, elder)
%             \item Physique
%             \item Weather
%             \item ...
%         \end{itemize}
%     \item Does diverse texts lead to diverse motion being generated? Measure the diversity of motion generated 
%         \begin{itemize}
%             \item An existing diversity metric exists in the field, has to do with euclidean distance between motion pairs. See the T2M-GPT\cite{zhang2023generating} paper for more details 
%             \item Can draw a chart of text diversity V.S. motion diversity
%         \end{itemize}
%     \item Experiment with different motion synthesis models to see if there is a difference in diversity and issues with confusion/hallucination.
%         \begin{itemize}
%             \item T2M-GPT \cite{zhang2023generating} (Used in original paper)
%             \item MotionDiffuse \cite{zhang2022motiondiffuse}
%              \item ReMoDiffuse \cite{zhang2022motiondiffuse}
%             \item MotionGPT \cite{jiang2023motiongpt}
%             \item HumanTOMATO \cite{humantomato} (additionally generate face and finger motions)
%             \item ...
%         \end{itemize}
%     \item Experiment with using motion style transfer methods to further increase the diversity of the generated motion
%         \begin{itemize}
%             \item Bandai-Namco-Research-Motiondataset (https://github.com/bandainamcoresearchinc/bandai-namco-research-motiondataset)
%             \item Style-ERD \cite{tao2022style}
%             \item Deep-motion-editing \cite{aberman2020unpaired}
%         \end{itemize}
%     \item Experiment with using mesh-based method (original paper uses skeleton-based) for generating sensor data. Uses various mesh model to represent people with different body shapes
%         \begin{itemize}
%             \item Mesh-based method \cite{Uhlenberg2022mesh}
%             \item Human Bodies in the Wild (Various body mesh for real people) \cite{Shapy:CVPR:2022}
%             \item Can then retarget the generated motion to various body meshes using Zhang \textit{et al.}'s work \cite{zhang2023skinned}
%         \end{itemize}
%     \item Motion-X \cite{lin2023motionx} is a recently released dataset on motion with caption, 4 times larger than HumanML3D \cite{Guo_2022_CVPR}. Can experiment with training motion synthesis model on this new dataset and see how the bigger dataset makes a difference.
%     \item How to combat the problem of hallucination/confusion, where motion synthesis models confuses closely related activities and verbs (see limitation of original paper for more detail)? This is a big problem as it introduces noise in the generated virtual IMU data, causing performance of downstream classifier to quickly plateau.
%         \begin{itemize}
%             \item Experiment with prompt weighting in diffusion based models(commonly used in text to image methods). Weight the activity related parts of text description more. 
%             \item Motion capation methods (e.g. MotionGPT \cite{jiang2023motiongpt}), to caption the generated motion, then use this caption to filter out bad motion (can input caption into LLM and ask if it is the right activity).
%         \end{itemize}

%     \item How to combat the problem of hallucination/confusion, where motion synthesis models confuses closely related activities and verbs (see limitation of original paper for more detail)? This is a big problem as it introduces noise in the generated virtual IMU data, causing performance of downstream classifier to quickly plateau.
%         \begin{itemize}
%             \item Experiment with prompt weighting in diffusion based models(commonly used in text to image methods). Weight the activity related parts of text description more. 
%             \item Motion capation methods (e.g. MotionGPT \cite{jiang2023motiongpt}), to caption the generated motion, then use this caption to filter out bad motion (can input caption into LLM and ask if it is the right activity).
%         \end{itemize}

%     \item How to generate activities that doesn't exist in the training dataset? Mentioned in discussion of original paper  
%         \begin{itemize}
%             \item Use LLM to breakdown activities into simpler movements (e.g. break bench press into lying down and pushing arm out). Then reconstruct the complex activity using SINC \cite{SINC:ICCV:2022} by feeding in the simpler movements. 
%         \end{itemize}
    
% \end{itemize}



% \noindent

==> sections/prompt_diversity/main.tex <==
\section{Measuring Diversity of textual descriptions and motion sequences}
\label{sec:diversity}
\thomas{Section 4 has an odd title. Remember we have two major contributions: the technical extensions and the experimental study. So, in section 4 (which will be section 3, sorry) we need to start with an overview of and motivation for these extensions / modifications. We could do this with an analysis of the original ISWC system that then leads to our extensions, which we then describe in individual subsections.}

\thomas{The problem with the text below is that we jump straight into the technical details without providing much (or any for that matter) justification / motivation. That does not go well for the overall flow.}

The primary goal of measuring the diversity for a set of text descriptions or motion sequences is to quantify the amount of useful information present in the set, and then utilize that to make a judgement about downstream performance without running the entire pipeline. The intuition is that if the diversity is high, then downstream models would be exposed to a broader range of data points during training. The models learn to make predictions on a wider variety of cases, thus improving the performance. Diverse training data also helps prevent the models from overfitting, since a limited dataset would lead to overexposure to a small section of the feature space. It is be helpful to have some practical, heuristic metrics which make it feasible to make an estimation of downstream performance at the time of generation itself, and diversity is computationally cheap to calculate. 

% The motivation for this stems from the time and compute resource limitations associated with generating virtual IMU data. Furthermore, the trend of higher amounts of virtual data leading to better downstream scores may not hold as the size of the virtual datasets increase. Under such circumstances, it is be helpful to have some practical, heuristic metrics which make it feasible to make an estimation of downstream performance at the time of generation itself. The diversity of the text descriptions and motion sequences is a suitable metric for this purpose since it is computationally cheap to calculate and is a good indicator of downstream classifier performance. 
\hyeok{The texts in these first two paragraphs are already mentioned multiple times in previous sections. So, please merge them, make it concise, and only keep what is new to the reader starting this section. Readers already waited enough to learn what method is actually used!}\amit{reduced content, brought down to one paragraph}

In order to calculate the diversity of the textual descriptions and the motion sequences, we generate embeddings for each prompt and sequence. This is because embeddings are effective in capturing information about the descriptions and the sequences in a quantitative, numerical format, and are thus more suitable for calculating metrics. The embeddings are generated as follows: 
\begin{itemize} 
    \item \textbf{Textual descriptions}: The text prompt are passed through sentence-transformers' all-mpnet-base-v2 model \cite{reimers-2019-sentence-bert, all-mpnet-base-v22024} on HuggingFace \cite{wolf2020huggingfaces} to generate embeddings for each prompt. This model is trained on a billion sentence pairs to capture the semantic information of its input text, and thus the embedding generated serves as a suitable representation of the sentence. 
    \item \textbf{Motion Sequences}: Each motion sequence is passed through a model trained on the HumanML3D dataset \hyeok{I suggest adding author name for all the citations}\cite{Guo_2022_CVPR} to generate the embeddings for the sequence. This model is drawn from the motion feature extractor trained in Guo et al. \cite{Guo_2022_CVPR}, and is commonly used in the community \cite{zhang2023generating}.
\end{itemize}
Overall, we compute two types of diversity - absolute diversity and comparative diversity. Note that these metrics are applicable on set of embeddings - this may correspond either to a set of embeddings generated from textual descriptions or to a set generated from motion sequences, the methods themselves are universally applicable to any collection of embeddings. Absolute diversity provides a quantitative measure for the amount of diverse information contained in a set, while comparative diversity showcases how much two sets differ in terms of their diversity. These are detailed further in the subsequent sections. 
\subsection{Absolute Diversity Metrics}
We use two methods to compute the absolute diversity of a set of embeddings - the standard deviation method and the centroid method. For both these metrics a higher value corresponds to a more diverse set, and vice versa. 
\subsubsection{Standard Deviation Metric}
The standard deviation method is based on the diversity metric highlighted in Lai et al. \cite{lai_diversity_nodate}. Treating embeddings as a vectors in a high-dimensional embedding space, the goal is to characterize the dispersion (the "spreadness") of a cluster of such vectors. If the cluster is assumed to be distributed as a multi-variate Gaussian, each isocontour will be shaped as an axis-aligned ellipsoid. The radii of the ellipsoid along each axis can be computed by calculating the standard deviation (i.e. the square root of variance) of the vectors in the cluster along each of the axes. Thus, computing the geometric mean of the radii would provide a generalized sense of the radius of the cluster, providing a sense of the diversity. Assuming the set of embeddings $S$ consists of $n$ embedding vectors, each of dimension $k$, the set can be formalized as $ S = \left\{ x_i \right\}_{i=1}^n \subset \mathbb{R}^k$. Thus, the standard deviations along an axis $ j \in [1, k] $ is computed as follows:
    \begin{equation}
        \sigma_j = \sqrt{\frac{\sum_{i=1}^{n}\left(x_i^j - \mu^j\right)^2}{n}} \text{, wherein }  \mu^j = \frac{\sum_{i=1}^{n}x_i^j}{n}  
    \end{equation}
    The final diversity score $M_{std}$ is calculated as:
    \begin{equation}
        M_{std} = \left( \prod_{j=1}^{k} \sigma_j \right)^{\frac{1}{k}}
    \end{equation}

\subsubsection{Centroid Metric}
    The centroid method is based on the methodology detailed in \cite{Duda2000}. Assume the set of embeddings $ S = \left\{ x_i \right\}_{i=1}^n \subset \mathbb{R}^k$, consisting of $n$ embedding vectors, each of dimension $k$. First, the centroid vector $x_{cent}$ of all the embedding vectors is calculated: 
    \begin{equation}
        x_{cent} = \frac{\sum_{i=1}^{n}x_i}{n}  
    \end{equation}
    The diversity score $M_{cent}$ is computed as the mean of the sum-squared distances of all the embedding vectors from the centroid vector:
    \begin{equation}
        M_{cent} = \frac{\sum_{i=1}^{n}\left(d(x_i, x_{cent})\right)^2}{n} \text{, wherein $d$ is the Euclidean distance }  d(x_i, x_{cent}) = \sqrt{\sum_{j=1}^{k}\left(x_i^j - x_{cent}^j\right)^2}
    \end{equation}
    The intuition for this method stems from the fact that the higher the diversity for a set of embeddings, the farther apart their vectors will be spread in the embedding space. As a result, the points will tend to be at a farther distance from the overall mean than for a less diverse set, and the centroid metric quantifies this aspect. 
    \hyeok{How do you pick the number of centroid?} \amit{there is just one centroid, which is the centroid of the entire set of embeddings}


\input{figure/algorithm}

\subsection{Comparative Diversity}\label{sec:comparative_diversity}
The text description generation process starts by generating an initial set of descriptions. Batches of textual descriptions are generated sequentially and are added to the growing set of pre-existing descriptions. If adding a new batch of textual descriptions improves the diversity of the pre-existing set, then continuing to further generate newer batches is well-motivated as it would contribute to the diversity of the motion sequences, leading to better downstream performance. On the contrary, if diversity does not improve, newer batches should not be generated. The goal of the comparative diversity is to quantify this change in diversity that occurs on adding a new batch to the pre-existing set. 
\hyeok{merge two paragraphs and make concise. Very redundant currently.} \amit{merged and reduced content}
Note that we make two implicit assumptions here:
\begin{itemize}
    \item Increased diversity in the set of text descriptions would correlate to increased diversity in the set of motion sequences generated.
    \item Higher diversity in the motion sequences would lead to better downstream model performance.
\end{itemize}
 Both these hypotheses are validated in the Section \ref{sec: diversity_predictor}

The comparative diversity between two sets of embeddings is computed using the Maximum Mean Discrepancy (MMD) test \cite{JMLR:v13:gretton12a}. MMD is kernel-based statistical test which indicates whether two given set of samples are the drawn from the same distribution or not. The higher the value, the farther the distributions of the two sets of samples. Thus, we interpret two embedding sets as being drawn from two distributions, and calculate the "distance" between these two distributions to serve as the difference in diversity. If the distributions of the two sets of embeddings are similar, they will have a similar diversity, and correspondingly the MMD value for the pair of sets will be lower. Further details about how the comparative diversity is utilized to halt the generation process is highlighted in the subsequent 


\subsection{Saturation Point Identification Algorithm}
\label{sec: algorithm}

Given the comparative diversity highlighted in the previous section, the goal is to utilize this metric in a manner wherein the generation of textual descriptions can be halted once the generated set of descriptions saturates. In order to determine this halting point, we propose the Saturation Point Identification algorithm, detailed in Algorithm \ref{alg:sat_point_ind}. Given a pre-existing set of textual descriptions $S$ of size $n$, the algorithm iteratively generates new batches of descriptions and tests if the adding the new batch to the pre-existing set alters the comparative diversity significantly. The size of the new batch is a percentage of the size of the pre-existing set, and is a tunable hyperparameter. Setting a higher value for the percentage would imply a coarser steps towards the saturation point. 

If adding the new batch alters the diversity substantially, then the diversity hasn't saturated yet, and the iteration continues. On the other hand if the diversity does not change meaningfully, it may be close to reaching saturation, and a counter is incremented to indicate this. Once the counter reaches a certain stopping value (set as a hyperparameter) the algorithm terminates. A higher value for this hyperparameter would lead to greater tolerance for saturation. 
\hyeok{Redundant text with previous sections. merge with previous sections and remove redundancy. I don't think a separate section for saturation is needed.} \amit{Removed repeated text in previous sections}

Note that for calculating the MMD between two sets of embeddings, the sets must have the same size. However, in this case we calculate the MMD between two sets of differing sizes (in Algorithm \ref{alg:sat_point_ind}, these are $S\_emb$ and $S\_emb + B\_emb$ respectively). In order to address these, we resample the smaller set (since resampling from a distribution does not alter it) until it has the same size as the larger set and then calculate the MMD. Note that this process of resampling is conducted multiple times, resulting in multiple values of MMD, and thus the function returns the mean score along with the standard deviation for MMD calculation ($MMD\_calculator$ function in Algorithm \ref{alg:sat_point_ind}). Our algorithm is evaluated in section \ref{sec: algo_eval}

==> sections/result/main.tex <==
\section{Result}
\thomas{We should not split 4 and 5. Make it one evaluation section. We also need experiments on more than one dataset.}
As shown in \autoref{tab:results}, the classifier trained on both real and virtual IMU data have improved performance compared to a classifier trained only real IMU data. The performance improvement is especially apparent when the reduced real IMU dataset is used. This shows the use of virtual IMU data for training is exceptionally beneficial when the amount of available real IMU data is limited.  

Furthermore, we observe that when data from all seven sensor locations are used, the classifier trained on only virtual IMU data outperforms the classifier trained on real IMU data. We find this surprising because the size of the virtual IMU dataset is less than 4\% of the size of the real IMU dataset. We attribute this performance imporvement to the diverse textual prompts that ChatGPT generated, which led to a diverse set of virtual IMU clips. Using such a diverse training data, the model learns to recognize the many variations of each activity. 

Overall, the two virtual IMU dataset led to classifiers with comparative performances with the exception of the classifier trained on only virtual IMU data from the forearm sensor. In this case, extracting joints' rotations by fitting the joints' positions to a SMPL model led to a better downstream classifier compared to using inverse kinematics for joints' rotations extraction. When inverse kinematics is used, the estimated rotations for joints farther in the kinematics chain will suffer from grater error due to error accumulation. Since the forearm joint is at the end of a kinematics chain, the error in the estimated forearm joint's rotations will be greater than that of the other joints, which leads to unrealistic virtual IMU data and in turn a worse classifier. However, we note that inverse kinematics is significantly faster than fitting to SMPL. On a RTX 2080ti, generating a five seconds clip of virtual IMU data takes five seconds using inverse kinematics, allowing real time generation, and one minute by fitting to SMPL.  





==> sections/system/main.tex <==
\section{IMUGPT: Language-Based Cross Modality Transfer for Sensor-Based Human Activity Recognition}

\input{figure/general_flow}

Language-based cross modality transfer approaches refer to methods that generate virtual IMU data from textual descriptions of activities, either from existing textual datasets or those generated by LLMs. \autoref{fig:general_flow} shows the general flow of language-based cross modality transfer methods, including two additional modules (shown in blue) that we propose in this work. \thomas{This sounds like there is a whole lot of such approaches, while in reality it is only us?}

An example of a language-based cross modality transfer method is the system recently introduced by Leng et al. \cite{leng2023generating}. This system consists of three major components as follows:
\hyeok{I think we can actually move this to the background section.}
\begin{enumerate}
\item \textbf{LLM}. \underline{What:} An LLM is used to generate diverse textual descriptions of a person performing a specified activity. \underline{Why:} Human activities are diverse in the real world, as the same activity can be performed in different ways by different people (e.g., a skinny teenager vs. a muscular athlete) and under different contexts (e.g., happily vs. sadly). To develop robust and generalizable HAR models capable of recognizing all these variations, it's essential to reflect this diversity in the training data. Generating diverse textual descriptions for activity performance is the first step toward ensuring the generated virtual IMU data accurately represents real-world diversity. Additionally, using an LLM for text generation automates and simplifies the process, eliminating the need to search for video data as required in video-based cross modality transfer approaches.
\item \textbf{Motion Synthesis}. \underline{What:} A motion synthesis model that takes in textual descriptions of the activity and converts them into three-dimensional human motion sequences. \underline{Why:} The motion synthesis model bridges the gap between text and human motion. To extract virtual IMU data, understanding how a person moves in three-dimensional space is essential. This is similar to how three-dimensional poses are estimated in video-based methods.
\item \textbf{Motion to IMU}. \underline{What:} A method to convert generated motion sequences into virtual IMU data, either biomechanically \cite{Yound2011imusim} or through neural networks \cite{Santhalingam2023asl, Li2023asl}. \underline{Why:} The virtual IMU data extracted from the motion sequences can be used to train a deployable HAR model, either alone or in conjunction with real IMU data.
\end{enumerate}
\thomas{Is the above verbatim from the ISWC paper?}\zikang{}

The pipeline has been evaluated on three standard HAR datasets, namely PAMAP2, RealWorld, and USC-HAD. \hyeok{these details are not needed. you can say "locomotion activities" with citations.}
It demonstrates that the extracted virtual IMU data leads to significant improvements in downstream classifier performance through small-scale evaluations. 
\hyeok{Move all text up to here to background section.}

In this work, we propose two additional modules, shown in blue in \autoref{fig:general_flow}, for language-based cross modality transfer as follows:

\begin{enumerate}
\item \textbf{Diversity Metric}. \underline{What:} A method to measure the diversity of textual descriptions and motion sequences generated by LLMs and motion synthesis models. See section \ref{sec:diversity} for more details. \underline{Why:} We hypothesize that the downstream model performance depends on the diversity of the virtual IMU data, as more diverse data can enhance model performance. With the proposed diversity metrics, we introduce a saturation point identification algorithm (section \ref{sec: algorithm}) that identifies the point at which generating additional textual descriptions no longer adds meaningful information to the existing pool of generated texts. This indicates a stopping point for generation. Automatically identifying when to stop data generation saves time and computing resources, which are not unlimited.
\item \textbf{Motion Filter}. \underline{What:} A pipeline that identifies and filters out motion sequences that do not accurately portray the specified activity. See section \ref{sec: motion_filter} for more details. \underline{Why:} The motion synthesis model does not always generate motion sequences that accurately portray a person performing the specified activity, as it can confuse closely related activities (e.g., climbing up stairs vs. climbing downstairs), resulting in irrelevant motion sequences. We hypothesize that irrelevant motion sequences will negatively impact the downstream classifier's performance by introducing noise. 
% Hence, we aim to filter out inaccurate motion sequences to ensure the accuracy of the extracted virtual IMU data. \hyeok{redundant.}
\end{enumerate}

\thomas{Sorry about flip-flopping but I now think the description of the original IMUGPT system should be part of related work. Sorry.}



% They provide prompts to ChatGPT \cite{openai2022gpt} in order to generate textual descriptions of activities present in popular HAR datasets like PAMAP2, RealWorld, and USC-HAD. The textual descriptions generated were input to a motion synthesis model -- T2M-GPT \cite{zhang2023generating} -- in order to generate a 3D motion sequence. With the help of inverse kinematics \cite{Yamane2003ik} and IMUSim -- an IMU simulation environment that converts joint rotations and translations into simulated IMU data \cite{Yound2011imusim}, they were able to generate virtual IMU data for activities in the aforementioned datasets.

% With this system, they were able to automate the process of generating textual descriptions as compared to the tedious search for the right videos presented in earlier systems. This reduced the overall time required to generate virtual IMU data. The textual descriptions generated with ChatGPT were highly diverse reflecting the diversity of real world activities. They further hypothesis that this diversity is translated into the generated virtual IMU data allowing for the development of a complex and generalizable model. 



% Leng et. al. \cite{leng2023generating} introduced the use of LLMs, motion synthesis, and signal processing for the generation of virtual IMU data. \autoref{fig:imugpt} presents and overview of the system. They provide prompts to ChatGPT \cite{openai2022gpt} in order to generate textual descriptions of activities present in popular HAR datasets like PAMAP2, RealWorld, and USC-HAD. The textual descriptions generated were input to a motion synthesis model -- T2M-GPT \cite{zhang2023generating} -- in order to generate a 3D motion sequence. With the help of inverse kinematics \cite{Yamane2003ik} and IMUSim -- an IMU simulation environment that converts joint rotations and translations into simulated IMU data \cite{Yound2011imusim}, they were able to generate virtual IMU data for activities in the aforementioned datasets.

% With this system, they were able to automate the process of generating textual descriptions as compared to the tedious search for the right videos presented in earlier systems. This reduced the overall time required to generate virtual IMU data. The textual descriptions generated with ChatGPT were highly diverse reflecting the diversity of real world activities. They further hypothesis that this diversity is translated into the generated virtual IMU data allowing for the development of a complex and generalizable model. The system used a standard Random Forest classifier and a DeepConvLSTM model by training the models on just the real IMU data, virtual data, and a combination of real and virtual data and were able to achieve relative improvements of  6.1\%, 7.7\%, and 1.7\% on PAMAP2, RealWorld, and USC-HAD datasets respectively.

% While the results present by Leng et. al. were promising, these were small-scale evaluations. A single LLM was used to generate just 50 textual descriptions for a total of 32 activities across 3 datasets. Furthermore, the experiments were conducted with motion sequences generated by just one motion synthesis model. In some instances, there were incorrectly generated motion sequences. When generating motion sequences for closely related activities, climbing upstairs and climbing downstairs for example, the motion synthesis model can often confuse the activities, causing incorrect motion sequences to be generated. The confusion also occurs when the input textual description, generated by LLMs, contains multiple verbs. In this case, the motion synthesis model may focus on the incorrect verb, generating incorrect motion sequences. Overall, there was a very small amount of virtual IMU data generated for the experiments. In this work, we tackle these limitations for experiments of a larger scale.

% With our added components, the overall pipeline is shown in \autoref{fig:general_flow}. The pipeline starts with the LLM generating textual descriptions of the input activity, which is then converted into motion sequences using the motion synthesis model. Our proposed motion filter will detect incorrectly generated motion sequences, and only the correctly generated motion sequences will be used to extract virtual IMU data. During the generation process, our proposed diversity metric is employed to determine the optimal moment to stop the generation process, ensuring efficiency and quality in the data produced. Afterwards, the generated virtual IMU data can be used to train a HAR model for deployment either alone or with real IMU data. 

==> tables/prompts.tex <==
\begin{table}
\centering
\caption{Example generated textual descriptions for 'climb up stairs' using various LLMs}
\vspace{-0.2cm}
\begin{tabular}{|>{\scriptsize}p{0.085\columnwidth}|>{\scriptsize}p{0.87\columnwidth}|}
\hline
% \textbf{Activity Name} & \textbf{Description} \\
% \hline
GPT-3.5 & A person places one foot on a step, holds onto the railing, and pulls themselves upward \textbf{;} \quad With a brisk pace, a person climbs the stairs effortlessly, displaying coordinated movements \textbf{;} \quad A man swiftly climbs the stairs, his body working in harmony to reach the top \textbf{;} \quad The climber exhibits grace and strength, swiftly ascending the stairs without hesitation \textbf{;} \quad A woman takes slow steps, gripping the handrail for support as she ascends \\
\hline
GPT-4 & A student with a heavy backpack trudges slowly upstairs \textbf{;} \quad A bride ascends a grand staircase, her dress flowing \textbf{;} \quad On tiptoes, the dancer ascends as if floating \textbf{;} \quad A tourist climbs historic stairs, stopping frequently to admire the view \textbf{;} \quad An athlete bounds up, using the workout for training \\
\hline
LLaMa 2 & A woman hikes up her backpack and begins the long climb up the stairs \textbf{;} \quad A person in a hurry takes the steps two at a time, their footsteps echoing urgently \textbf{;} \quad A man climbs the stairs, his eyes fixed on the landing above, lost in thought \textbf{;} \quad A person carefully makes their way down the stairs, holding onto the rail for support \textbf{;} \quad A woman in heels carefully makes her way up the stairs \\
\hline
Palm 2 (Bard) & A person climbs the stairs, their face smiling \textbf{;} \quad A person climbs the stairs, their face frowning \textbf{;} \quad A dog climbs the stairs, its tail wagging with anticipation \textbf{;} \quad A cat climbs the stairs, its eyes shining with excitement \textbf{;} \quad A life climbs up the stairs, one step at a time \\
\hline
Gemini & A woman walks up the stairs while reading a book \textbf{;} \quad A woman climbs the stairs while doing the lindy hop \textbf{;} \quad Woman climbs stairs with determination, despite her exhaustion \textbf{;} \quad Woman climbs stairs quickly, heart pounding in her chest \textbf{;} \quad A bee buzzes up the stairs, its body covered in pollen \\
\hline
\end{tabular}
\label{tab:prompts}
\end{table}


